ApSense: Data-driven Algorithm in PPG-based Sleep Apnea Sensing

Detecting obstructive sleep apnea (OSA) is essential for diagnosing and managing sleep health. Traditionally, this involves clinical settings with hardly accessible processes. We propose that the automated detection of OSA events is achievable using features extracted from fingertip photoplethysmography (PPG) signals combined with modern deep learning (DL) techniques. Utilizing two benchmark data sets with extensive PPG recordings, we introduce ApSense, a DL model designed for the OSA event onset recognition from PPG features. ApSense presents a custom neural architecture and domain-specific feature extraction from PPG waveforms. We benchmark it against the state-of-the-art (SOTA) algorithms, including RRWaveNet, PPGNetSA, AIOSA, DRIVEN, and LeNet-5. In our evaluations, ApSense demonstrated improved sensitivity, specificity, and area under the receiver operating characteristic (AUROC) on the test data sets. Furthermore, an ablation study highlighted strategic customizations of ApSense, enhancing its performance and adaptability to different data sets. ApSense demonstrates high reliability, as its outstanding results were confirmed even in high-variance data sets. By detecting OSA events, ApSense enables the estimation of the predicted apnea-hypopnea index (pAHI), which can be used for prescreening individuals for sleep apnea in a low-cost setup. ApSense shows the potential for the PPG-based OSA detection and clinical applications for prescreening in the future.

==> content/Extensions.tex <==
\section{Extensions}


\subsection{Human-Machine Collaboration}
\label{sec:med:H}

Recent work in the field of AI in sleep medicine, \cite{bam} presented a practical scenario to fine-tune the pre-trained model to be personalized for an unseen patient by allowing clinicians (humans) to manually annotate sleep stages within a few percent of the whole night data and let the machine (AI or DL model) to predict the rest. In summary, they report the predicted hypnogram with up to 89\% accuracy against the clinician, which is a convincingly promising application of DL techniques to assist time-consuming tasks such as screening the whole night sleep data, including multiple time series.

This paper addresses the same issue while enabling a fast and costless adaptation of the model to each particular subject through a simple fine-tuning technique. Available on DL models, we fine-tune the model using a few annotations of apnea events on the signals obtained from the unseen patient. 

For each test subject, we reserve a fraction of samples from that subject for the fine-tuning and update two of the DL models (Mini-RRWaveNet and DSepNet) with the same learning rate for $10$ epochs with a batch size of $64$. We also vary the fractions to observe the cost-performance tradeoff. 

In this paper, an attempt with longer fine-tuning fails to show significant improvement, while a shorter trial with less than $10$ terminates before the model converges. One could alternatively apply an early stopping technique to avoid underfitting and overfitting when the number of labeled unseen samples is highly available – an expensively satisfied requirement. 


While the apnea detection performance results in Table \ref{table:exp3} overemphasize the sensitivity, in this experiment, the accuracy improves by up to an absolute 20\% with a simple fine-tuning technique. Measures in Table \ref{table:exp4} report the detection performance with varying ratios of test samples utilized for model fine-tuning, revealing a significant improvement in all measures. The sensitivity is relatively modest compared to Table \ref{table:exp4} in exchange for the enhanced specificity. 

With $<$10\% of the test samples, fine-tuning can negatively impact the prediction, as pointed out via performance drop when only 5\% of the test samples are used. Training with more abundant samples helps the DL model fit better to the unseen distribution and thus yields higher detection accuracy. 

\begin{figure}
  \center
  \includegraphics[width=0.75\columnwidth, trim=1.9cm 0 2cm 1cm, clip]{figure/scatter_finetune/DSepNet_0.png}
  \includegraphics[width=0.75\columnwidth, trim=2cm 0 2cm 1cm, clip]{figure/scatter_finetune/DSepNet_20.png}
  \caption{Correlation plots between eAHI and DSepNet's pAHI without (top) and with (bottom) fine-tuning in the two datasets, MESA and HeartBEAT. Without fine-tuning, the model overfits the sensitivity, which results in the weak pAHI-sAHI correlation and the overestimation of AHI.}
  \label{fig:scatter_finetune}
\end{figure}



\subsection{Overnight AHI Estimation}

Clinicians and researchers in sleep studies classify the severity of OSA into three categories using predefined AHI thresholds. Figure \ref{fig:AHI}, for example, shows the distribution of OSA severity of the subjects from the two datasets. For each severity class, it is recommended to provide particular treatment for better management toward recovery \cite{goyal2017obstructive}. OSA patients with AHI above 15 should receive continuous positive airway pressure (CPAP) therapy to reduce such risks, including loss of productivity and road accidents.

Recognition of apnea events during the sleep test directly relates to the calculation of AHI, which equals the number of apnea events per unit of time, commonly in hours. In this paper, we generate a label for each of the 60s signal windows, identifying the presence of the apnea event. 

Using our feature extraction and event annotation method, a window can be discarded due to extreme noise artifacts. Any apnea events that coexist in a single window count as one. Missing counts of apnea events may occur in our dataset. Alternatively, we propose an estimated measure, \emph{sampled AHI} or sAHI, to represent each subject's AHI compatible with our data preparation methodology. As two consecutive 60s windows overlap by 50\% or 30 seconds, we define sAHI per hour as:
\begin{equation}
    \text{sAHI} = \frac{\text{number of apneic windows}}{30 \times \text{number of total windows} + 30} \times 3600 
\end{equation}

Similarly, the predicted AHI, or pAHI per hour, can be calculated from the prediction values.
\begin{equation}
    \text{pAHI} = \frac{\text{number of apneic predictions}}{30 \times \text{number of total windows} + 30} \times 3600 
\end{equation}
where a prediction is made per window. Ideally, we would have $\text{sAHI} = \text{pAHI}$ when the model always predicts correctly. The correlation between both measures is shown in the next section. 

%\input{table/table_exp1}

Plots in Figure \ref{fig:scatter_finetune} show the correlation between sAHI and pAHI per subject, calculated based on the ground truth labels and the model predictions of the test samples from the two datasets. Without fine-tuning, it is hard to convince there is a strong correlation between the two measures due to poor recognition performance. Especially in the HeartBEAT dataset which the models overfit to positive samples, it is easily noticeable that pAHI is overestimating the sAHI, which may cause too many unnecessary false alarms in practice.

After model fine-tuning, although the overestimation does not completely vanish, the Pearson coefficient $r$ between sAHI and pAHI raises to $0.794$ and $0.654$ in the MESA and HeartBEAT dataset, respectively. This implies the feasibility of using pAHI as an indirect measure of OSA severity, where sleep patient monitoring can be done in a semi-manned scheme. 


%\input{table/table_exp3}
%\input{table/table_exp4}












==> content/RESULTS-II.tex <==
\section{Experimental results}
\label{sec:results}


\subsection{\textcolor{red}{Experiment I: ApSense optimization}}

As detailed earlier, ApSense incorporates the multiple RVarDsepBlock (spatio-temporal blocks), BCNN, and LSTM with VDO. We initially optimized ApSense by removing the specific components separately and providing insights into the distinct contributions of each component to the overall system.

We assessed the classification performance within a subject-independent framework to identify the most effective ApSense configuration for recognizing OSA events across two datasets: MESA and HeartBEAT, as illustrated in \autoref{table:exp_prove}. 

\textcolor{red}{In the HeartBeat dataset, with the presence of stacked RVarDSepBlock (N=4), removing BCNN disturbed the fine-tuned balance between specificity and sensitivity. This imbalance was rectified upon reintroducing the BCNN; however, the AUROC score remained low. The incorporation of both VDO along with BCNN resulted in enhancement, yielding an approximate 7\% improvement in AUROC.}

\textcolor{red}{Unlike HeartBEAT dataset, the MESA dataset exhibited contrasting performance when using those components. Excluding BCNN resulted in improvements across all metrics—approximately 3\% for accuracy, 4\% for F1-score, 8\% for sensitivity, 2\% for specificity, and 6\% for AUROC. Similarly, removing VDO also led to a slight increase in those metrics, compared to combining both of these components.} 

\textcolor{red}{The impact of employing varying numbers of the stacked RVarDsepBlock (N) for each feature map size was more pronounced in the case of the HeartBEAT dataset. Applying fewer or more than four blocks led to a noticeable decline in Apsense's performance, whereas the MESA dataset exhibited a more tolerant response to changes in the block numbers.}

\textcolor{red}{
The results indicate that the most effective ApSense was the difference across the two datasets.}




\subsection{\textcolor{red}{Experiment II: Benchmarking ApSense against baseline methods for OSA event detection}}

\textcolor{red}{We selected the best ApSense configuration considering the highest AUROC across two datasets. As illustrated in \autoref{Experiment_I}. 

\In the MESA dataset, the classification results of the methods were close to each other. PPGNetSA exhibited superior performance in nearly all metrics, such as accuracy, F1-score, and specificity. However, MiniAIOSA demonstrated a more balanced trade-off between sensitivity and specificity, ultimately yielding the highest AUROC.} 

\textcolor{red}{Despite the apparent effectiveness of these baseline models compared to ApSense, it is essential to highlight a significant imbalance in results between sensitivity and specificity in the HeartBEAT dataset for those baseline methods, including MiniRRWaveNet. There were substantial differences with gaps in these metrics, approximately 47\%, 29\%, and 51\% for MiniRRWaveNet, PPGNetSA, and MiniAIOSA, respectively. In contrast, ApSense showed the ability to fine-tune this balance, reducing the gap to only about 14\%, and achieving the best AUROC compared to the others}



\subsection{\textcolor{red}{Experiment III: Overnight AHI Estimation}}
\textcolor{red}{In this experiment, we applied ApSense for further estimation of AHI. This estimation involved dividing the total predicted apnea events by the overall duration of sleep. To assess its reliability in AHI prediction, we plotted the correlation between sAHI and pAHI per subject. The sAHI was calculated in \autoref{Overnight AHI Estimation}, as ground truth labels while pAHI was derived from the predicted AHI by our proposed methods for each window.} 

\textcolor{red}{ As illustrated in \autoref{fig:new_correlation AHI}, the pAHI exhibited a significant positive correlation with the sAHI across two datasets, particularly in the HeartBEAT dataset, resulting in a higher correlation coefficient (\textit{r}). The result underscores the reliable evaluation of AHI using pAHI derived from our proposed methods.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{\textcolor{red}{Experiment I: Benchmarking ApSense against baseline methods for OSA event detection}}


\begin{table*}
\centering
\tiny
\caption{The classification results for apnea event recognition, comparing ApSense to baseline models across two datasets. The results are presented as the average percentage $\pm$ standard deviation (SD).}
\label{Experiment_I}
\resizebox{\textwidth}{!}{%
    \input{new_tables/Experiment_I}
    }
\end{table*}



\begin{table*}
\centering
\tiny
\caption{Ablation study: The performance of ApSense system by removing certain components to understand each component's contribution to the overall system}
\label{Ablation study}
\resizebox{\textwidth}{!}{%
    \input{new_tables/Ablation study}
    }

\begin{tablenotes}
  \scriptsize
  \item  \textbf{Abbreviations:} N: Number of stacked RVarDsepBlock for each feature map size of 64, 32, 16, and 8, as illustrated in \autoref{fig:model}.  VDO: LSTM variational dropout. BCNN: Branch convolutional neural network
\end{tablenotes}
\end{table*}


\textcolor{red}{As illustrated in \autoref{Experiment_I}, we assessed the classification performance within a subject-independent framework to identify the most effective method for recognizing OSA events on two datasets: MESA and HeartBEAT. The performances of all methods were comparable in various metrics.} 

\textcolor{red}{In the MESA dataset, the classification results of the methods were close to each other. PPGNetSA exhibited superior performance in nearly all metrics, such as accuracy, F1-score, and specificity. However, MiniAIOSA demonstrated a more balanced trade-off between sensitivity and specificity, ultimately yielding the highest AUROC.} 

\textcolor{red}{Despite the apparent effectiveness of these baseline models compared to ApSense, it is essential to highlight a significant imbalance in results between sensitivity and specificity in the HeartBEAT dataset for those baseline methods, including MiniRRWaveNet. There were substantial differences with gaps in these metrics, approximately 47\%, 29\%, and 51\% for MiniRRWaveNet, PPGNetSA, and MiniAIOSA, respectively. In contrast, ApSense showed the ability to fine-tune this balance, reducing the gap to only about 14\%, and achieving the best AUROC compared to the others.}






\subsection{\textcolor{red}{Experiment II: Overnight AHI Estimation}}



\begin{figure}
  \center
  \includegraphics[width=\columnwidth]{figure/scatter_finetune/DSepNet15.png}
  \caption{Correlation between predicted AHI (pAHI) and sampled AHI (sAHI), with pAHI calculated from the predicted apnea events by ApSense}

  \label{fig:new_correlation AHI}
\end{figure}



\textcolor{red}{In this experiment, we applied ApSense for further estimation of AHI. This estimation involved dividing the total predicted apnea events by the overall duration of sleep. To assess its reliability in AHI prediction, we plotted the correlation between sAHI and pAHI per subject. The sAHI was calculated in \autoref{Overnight AHI Estimation}, as ground truth labels while pAHI was derived from the predicted AHI by our proposed methods for each window.} 

\textcolor{red}{ As illustrated in \autoref{fig:new_correlation AHI}, the pAHI exhibited a significant positive correlation with the sAHI across two datasets, particularly in the HeartBEAT dataset, resulting in a higher correlation coefficient (\textit{r}). The result underscores the reliable evaluation of AHI using pAHI derived from our proposed methods.}










\subsection{\textcolor{red}{Ablation study}}

\textcolor{red}{Conducting an ablation study on ApSense involves evaluating its performance through the targeted removal of specific components, providing insights into the distinct contributions of each component to the overall system. As detailed earlier, ApSense incorporates the multiple RVarDsepBlock (spatio-temporal blocks), branch CNN, and LSTM variational dropout. \autoref{Ablation study} presents the results of the ablation experiments, wherein each of these components is separately removed.}

\textcolor{red}{In the HeartBeat dataset, with the presence of four stacked spatial-temporal blocks, removing the branch CNN disturbed the fine-tuned balance between specificity and sensitivity. This imbalance was rectified upon reintroducing the branch CNN; however, the AUROC score remained low. The incorporation of both LSTM variational dropouts along with the branch CNN resulted in enhancement, yielding an approximate 7\% improvement in AUROC.}

\textcolor{red}{Unlike the HeartBEAT dataset, the MESA dataset exhibited contrasting performance when using those components. Excluding the branch CNN resulted in improvements across all metrics—approximately 3\% for accuracy, 4\% for F1-score, 8\% for sensitivity, 2\% for specificity, and 6\% for AUROC. Similarly, removing LSTM variational dropout also led to a slight increase in those metrics, compared to combining both of these components.} 

\textcolor{red}{The impact of employing varying numbers of stacked RVarDsepBlock (N) for each feature map size was more pronounced in the case of the HeartBEAT dataset. Applying fewer or more than four blocks led to a noticeable decline in Apsense's performance, whereas the MESA dataset exhibited a more tolerant response to changes in the block numbers.}

\textcolor{red}{
The results indicate that leveraging the advantages of ApSense's component depends on the specific data utilized.}







\iffalse
Recently, there has been a growing interest in applying spatiotemporal neural networks for biopotential applications. This motivates us to design Apsense by using multiple RVarDSepBlock blocks with increasing depth (Fn; n = ุ64, 32, 16, 8). Each depth level (n) is repeatedly stacked 4 times to capture different levels of features to extract spatial and temporal information in multi-resolution simultaneously, as drawn in Figure [XXX]. 

Each RVarDSepBlock has a residual depthwise convolution guided by \cite{9879745} with batch normalization and ReLu activation followed by a pointwise convolution and LSTM module, applying a variational dropout to mitigate overfitting  \cite{gal2016theoretically}. All of these are followed by average pooling. The output of these multiple RVarDSepBlock blocks is then used as an input to two branches - a regular 1-D convolution and a 1x1 convolution. The 1x1 convolutional layer is used to reduce the time dimension. This convolution treats each time stamp as a separate channel - acting as a non-time invariant filter to complement the time-invariant 1-D convolution. Batch normalization and ReLU activation are used for both branches. Finally, the input of these convolutions is passed to two fully connected layers to get the prediction.
\fi








\subsection{ApSense}
ApSense comprises three primary components: (i) a spatiotemporal block, (ii) a branch convolutional neural network or BCNN, and (iii) a dense, fully connected layer, as illustrated in \autoref{fig:model}. The spatiotemporal block consists of a series of RVarDSepblocks stacked arbitrarily, each defined by a fixed sequence of a number filters ($F_{n}$) = 64, 32, 16, and 8, repeated $M$ times. Each RVarDSepBlock includes a residual depthwise separable 1D-convolution splitting the computation into two steps: depthwise and point-wise convolutions, followed by batch normalization, ReLU, and unidirectional LSTM module. The LSTM module incorporates a variational dropout, masking input dropout = 0.1. The output channel in this layer is updated to the sum of the input (in\_ch) and output (out\_ch) channels. After each RVarDSepblock, an average pooling operation is applied to reduce size. Subsequently, the final output of RVarDSepblock is fed into two parallel convolutional branches: one being regular 1-D convolution and the other 1x1 convolution. Both convolutions are followed by batch normalization and ReLU activation functions. Afterward, the outputs of these branches are flattened and concatenated before being passed through two fully connected layers to generate the OSA onset recognition.

\subsection{MiniAIOSA}
MiniAIOSA is modified from AIOSA architecture \cite{benjafield2019estimation}, which originated for ECG-based OSA onset event recognition to be compatible with PPG. It consists of (i) three multiple separable CNN blocks (Multi-SCNN Block), (ii) an LSTM module, and fully connected layers, as presented in \autoref{fig:model}. Each Multi-SCNN Block has four SCNN blocks arranged in a series. Each SCNN block comprises the residual depthwise separable 1D-convolution (incorporating depthwise and pointwise convolutions) with a dilation, followed by batch normalization, ReLU activation, and concluding spatial dropout. Within each SCNN block, the number of filters ($F_{n}$) = 16 and a kernel size ($k$) = 3, while the number of dilations ($d$) varies. We let $d = L$ where $L$ is set to 1, 2, 4, 8 corresponding to their arrangement. The spatial dropout ($D$) is defined differently than is $D_{i}$ where $i$ is the series of the three multiple separable CNN blocks and is set to 0.2, 0.1, and 0.3, respectively. The average pooling operation is employed at the end of each Multi-SCNN block. The output of the multi-separable CNN module is then fed into the bidirectional LSTM module with the variational dropout (VDO), utilizing input dropout = 0.1. The output of this module is passed to two fully connected layers to predict OSA events.




\subsection{MiniAIOSA}%%% 6/02/66
MiniAIOSA is modified from AIOSA architecture \cite{benjafield2019estimation}, which originated for ECG-based OSA onset event recognition to be compatible with the PPG waveform feature. It consists of (i) three multiple separable CNN blocks (Multi-SCNN Block), (ii) an LSTM module, and fully connected layers, as presented in \autoref{fig:model}. Each Multi-SCNN Block has four SCNN blocks arranged in a series. Each SCNN block comprises the residual depthwise separable 1D-convolution (incorporating depthwise and pointwise convolutions) with a dilation, followed by batch normalization, ReLU activation, and concluding spatial dropout. Within each SCNN block, the number of filters ($F_{n}$) = 16 and a kernel size ($k$) = 3, while the number of dilations ($d$) varies. We let $d = L$ where $L$ is set to 1, 2, 4, 8 corresponding to their arrangement. The spatial dropout ($D$) is defined differently than is $D_{i}$ where $i$ is the series of the three multiple separable CNN blocks and is set to 0.2, 0.1, and 0.3, respectively. The average pooling operation is employed at the end of each Multi-SCNN block. The output of the Multi-SCNN Block is then fed into the bidirectional LSTM module with the variational dropout (VDO), utilizing input dropout = 0.1. The output of this module is passed to two fully connected layers to predict OSA events. Originally, AIOSA used window-wise output concatenation to turn the OSA prediction with a dense layer size of 60. Here, we adapt the number of dense size 1 for OSA prediction per window.  




\subsection{PPGNetSA}
\textcolor{red}{The PPGNetSA model presents the advanced version of the original EEGNet architecture \cite{lawhern2018eegnet} toward applications of PPG instead of EEG. The PPGNetSA incorporates three blocks: a self-attention mechanism, a branch block, and a depthwise convolution block. Each block is specifically designed to improve the process of extracting and analyzing spatial and temporal features from PPG signals. The input signal is handled through the model using two parallel convolutional layers in the branch block. One of these layers uses a kernel size, which is half the size of the window, to extract features at a broad frequency. The other layer implements a kernel size (k) = 3 for the transient feature. This setup promises a balanced representation of both long-term and short-term signal features, referred to as batch normalization and ReLU activation. It supports a framework for non-linear and normalized processing. Enhancing spatial features across PPG channels, ELU activation, and average pooling enables the subsequent depthwise convolution block to extract crucial spatial information.
The PPGNetSA introduces an innovative approach by decomposing the input feature map into three vectors using convolutional layers and a self-attention mechanism. This enables the model to dynamically weight features according to their mutual relevance, determined by attention scores and softmax normalization. This attention-based refinement enables the model to effectively prioritize important signal patterns by selectively enhancing significant features. PPGNetSA presents a practical approach for analyzing PPG signals by combining attention mechanisms and convolutional processing. This integration optimizes the prioritization and extraction of signal features, resulting in improved accuracy and interpretability.}





%Tanut
the convolutional neural network architecture of EEGNet \cite{lawhern2018eegnet}. To detect apnea events, PPGNetSA is a refined model designed for PPG signal analysis. By modifying the architecture of EEGNet, which allows for efficient training with limited data and the extraction of meaningful features, it becomes feasible to handle PPG features. PPGNetSA applies a unique approach by integrating a branch block utilizing a convolutional layer to enable variable kernel sizes, depthwise convolution to extract features specific to separate channels, and spatial convolutions with groupings to accomplish detailed feature mapping. For the purpose of apnea detection in PPG features, it implements an attention mechanism via linear transformations and a softmax operation to refine extracted and represented features.}

\textcolor{green}{Three customized blocks compose the PPGNetSA model. For a comprehensive feature analysis, the branch block convolutional layer (BCNN) utilizes two parallel convolutional layers. The filter size is half the window size, which accounts for broad frequency features. The kernel size ($k$) and stride ($s$) are both set to 3. Batch normalization and ReLU activation are also integrated. The spatiotemporal convolutional neural network block extracts particular spatial and temporal information through the use of batch normalization, average pooling and ELU activation on a depthwise convolutional layer, with filter sizes ($F_{n}$) of 256. Then followed with a convolutional layer, with filter sizes ($F_{n}$) of 256 and 128 for each. In conclusion, for the detection of apnea events, the self-attention mechanism employs attention scores and softmax normalization to dynamically weight signal features by using the convolutional layer, with filter sizes ($F_{n}$) of 128.}

==> new_tables/Experiment_I.tex <==
{\renewcommand{\arraystretch}{0.88}
\begin{tabular}{@{}llccccc@{}}

\toprule[0.2em]
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & 

\multicolumn{4}{c}{\textbf{Metrics}} \\
\cmidrule[0.1em]{3-7}
& & Accuracy & Macro F1 & Sensitivity & Specificity &AUROC\\ 

\midrule[0.1em]


\multirow{6}{*}{\emph{MESA}}

&RRWaveNet &69.81 $\pm$ 0.84 &61.44 $\pm$ 0.45 &61.09 $\pm$ 4.88	&71.89 $\pm$ 2.11	&71.87 $\pm$ 1.53 \\


& PPGNetSA  &71.39 $\pm$ 1.11	&61.94 $\pm$ 1.36	&56.56 $\pm$ 3.50	&74.93 $\pm$ 1.56	&72.13 $\pm$ 2.01 \\


&AIOSA (Unimodal variant)  &71.86 $\pm$ 1.43	&64.52 $\pm$ 0.88	&63.46 $\pm$ 7.35  &73.85 $\pm$ 3.24	&75.88 $\pm$ 2.36 \\

&LeNet-5  &67.60 $\pm$ 6.81  &54.88 $\pm$ 5.09  &50.80 $\pm$ 25.61	&71.49 $\pm$ 14.34	&64.62 $\pm$ 7.44 \\

&DRIVEN &73.93 $\pm$ 2.74 &67.48 $\pm$ 3.08 &77.17 $\pm$ 8.63 &73.26 $\pm$ 2.37	&82.45 $\pm$ 5.40 \\

& ApSense   & \textbf{75.10 $\pm$ 2.70}	&65.73 $\pm$ 4.84	&61.71 $\pm$ 17.41 & \textbf{78.46 $\pm$ 1.62}	&77.64 $\pm$ 7.93 \\


\midrule[0.1em]






\multirow{6}{*}{\emph{HeartBEAT}} 

&RRWaveNet  &51.33 $\pm$ 3.45	& 47.04 $\pm$ 2.17  &85.76 $\pm$ 3.92	 &45.96 $\pm$ 4.49	 &69.46 $\pm$ 2.23 \\


&PPGNetSA  &54.78 $\pm$ 2.64	 &49.09 $\pm$ 1.55	&79.77 $\pm$ 2.03	&50.86 $\pm$ 3.31	&69.28 $\pm$ 1.82 \\


&AIOSA (Unimodal variant)  &47.95 $\pm$ 2.34	&45.01 $\pm$ 1.65	&92.95 $\pm$ 2.17	&40.49 $\pm$ 2.91	& 70.20 $\pm$ 2.15 \\

&LeNet-5  &60.74 $\pm$ 3.67	&51.70 $\pm$ 1.49	&65.55 $\pm$ 5.49 &59.90 $\pm$ 4.98	&68.03 $\pm$ 1.77 \\

&DRIVEN  &55.52 $\pm$ 1.44	&49.13 $\pm$ 1.04	&74.85 $\pm$ 3.66	&52.53 $\pm$ 1.37	&67.54 $\pm$ 2.32 \\

& ApSense  &\textbf{62.31 $\pm$ 3.06}	 &54.12 $\pm$ 3.55	&74.87 $\pm$ 10.91	&\textbf{60.26 $\pm$ 3.35}	&\textbf{74.35 $\pm$ 6.46} \\

\bottomrule[0.2em]
\end{tabular}








==> table/hyperparameter.tex <==
\begin{table}[t]
\centering
\caption{Hyperparameter Search Space for ML Models}
\label{tab:mlhyper}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cll}
    \toprule[0.2em]
    \textbf{Model} & \textbf{Parameter} & \textbf{Values} \\
    
    \midrule[0.1em]
    
    \multirow{4}{*}{SVM} & Kernel & Linear, RBF \\
    & $C$ & $0.001,~0.01,~0.1,~10,~50,~100$ \\
    & $\gamma$ & $0.0001,~0.001$ \\
    & Maximum number of iterations & $10000$ \\
    
    \midrule[0.1em]

    \multirow{2}{*}{RF} & Maximum depth & $3,~5,~10$ \\
    & Minimum sample split & $2,~5,~10$ \\
    
    \midrule[0.1em]

    \multirow{3}{*}{XGB} & Number of estimators & $50,~100,~200$ \\
    & Maximum depth & $3,~6$ \\
    & Learning rate & $0.05,~0.1,~0.2$ \\
    
    \bottomrule[0.2em]

\end{tabular}
}
\end{table}

==> table/table_exp1.tex <==
\begin{table}[!t]
\caption{Apnea Event Recognition Performance by Model}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llcccc}

\toprule[0.2em]
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & 
\multicolumn{4}{c}{\textbf{Metrics}} \\
\cmidrule[0.1em]{3-6}
& & Accuracy & Macro F1 & Sensitivity & Specificity \\ 

\midrule[0.1em]

\multirow{6}{*}{\emph{MESA}} & SVC & 47.47 $\pm$ 3.07 & 40.20 $\pm$ 1.91 & 60.04 $\pm$ 3.36 & 45.98 $\pm$ 3.51\\ 
& RF & 62.58 $\pm$ 1.54 & 49.96 $\pm$ 1.36 & 58.53 $\pm$ 3.32 & 63.07 $\pm$ 1.88\\ 
& XGB & 89.44 $\pm$ 0.60 & 47.26 $\pm$ 0.17 & 0.05 $\pm$ 0.04 & 100.00 $\pm$ 0.00\\ 
\cmidrule[0.05em]{2-6}
& Mini-RRWaveNet & 71.66 $\pm$ 1.11 & 56.96 $\pm$ 0.40 & 62.77 $\pm$ 4.28 & 72.70 $\pm$ 1.52\\ 
& DSepNet & 71.08 $\pm$ 0.76 & 57.10 $\pm$ 0.71 & 66.43 $\pm$ 3.94 & 71.63 $\pm$ 0.81\\ 
& DSepEmbedder & 63.31 $\pm$ 1.49 & 49.22 $\pm$ 1.16 & 50.34 $\pm$ 2.67 & 64.86 $\pm$ 1.89 \\ 

\midrule[0.1em]

\multirow{6}{*}{\emph{HeartBEAT}} & SVC & 71.23 $\pm$ 3.04 & 49.46 $\pm$ 0.79 & 39.13 $\pm$ 5.31 & 73.72 $\pm$ 3.50 \\ 
& RF & 46.09 $\pm$ 2.65 & 39.45 $\pm$ 1.51 & 90.51 $\pm$ 1.39 & 42.61 $\pm$ 3.05 \\ 
& XGB & 92.77 $\pm$ 0.64 & 48.13 $\pm$ 0.17 & 0.00 $\pm$ 0.00 & 100.00 $\pm$ 0.00 \\ 
\cmidrule[0.05em]{2-6}
& Mini-RRWaveNet & 45.84 $\pm$ 2.69 & 39.33 $\pm$ 1.55 & 91.20 $\pm$ 2.37 & 42.30 $\pm$ 3.04 \\ 
& DSepNet & 46.35 $\pm$ 2.42 & 39.65 $\pm$ 1.51 & 90.67 $\pm$ 3.32 & 42.91 $\pm$ 2.68 \\ 
& DSepEmbedder & 70.94 $\pm$ 1.64 & 49.80 $\pm$ 0.60 & 41.97 $\pm$ 0.29 & 73.19 $\pm$ 1.60 \\ 

\bottomrule[0.2em]
\end{tabular}
}
\label{table:exp1}
\end{table}

==> table/table_exp2.tex <==
\begin{table}[!t]
\caption{Efficiency of the Event Annotation Methods}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llcccc}

\toprule[0.2em]
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & 
\multicolumn{4}{c}{\textbf{Improvement by Absolute Percentage}} \\
\cmidrule[0.1em]{3-6}
& & Accuracy & Macro F1 & Sensitivity & Specificity \\ 

\midrule[0.1em]

\multirow{4}{*}{\emph{MESA}} & RF & -0.61 & 0.02 & 2.95 & -1.05 \\
& XGB & 0.03 & 0.04 & 0.04 & 0.00 \\
& Mini-RRWaveNet & 0.36 & 0.66 & 2.43 & 0.12 \\
& DSepNet & 0.38 & 0.87 & 3.79 & -0.02 \\

\midrule[0.1em]

\multirow{4}{*}{\emph{HeartBEAT}} & RF & -1.96 & -1.14 & 3.03 & -2.32 \\
& XGB & 0.05 & 0.02 & 0 & 0 \\
& Mini-RRWaveNet & 0.82 & 0.45 & -1.05 & 0.99 \\
& DSepNet & -1.68 & -0.79 & 4.35 & -2.17 \\

\bottomrule[0.2em]
\end{tabular}
}
\label{table:exp2}
\end{table}

==> table/table_exp3.tex <==
\begin{table}[!t]
\caption{Apnea Event Recognition (per window or every 60 seconds) Performance by Model with Class Balancing and Data Augmentation Techniques}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llcccc}

\toprule[0.2em]
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & 
\multicolumn{4}{c}{\textbf{Metrics}} \\
\cmidrule[0.1em]{3-6}
& & Accuracy & Macro F1 & Sensitivity & Specificity \\ 

\midrule[0.1em]

% \multirow{6}{*}{\emph{MESA}} & SVC & 40.09 $\pm$ 7.61 & 38.51 $\pm$ 6.33 & \textbf{74.01 $\pm$ 13.15} & 32.25 $\pm$ 12.07 \\ 
% & RF & 60.20 $\pm$ 1.64 & 54.26 $\pm$ 1.31 & 63.48 $\pm$ 4.61 & 59.48 $\pm$ 2.85 \\ 
% & XGB & 67.73 $\pm$ 0.69 & 58.38 $\pm$ 0.42 & 53.46 $\pm$ 4.26 & 71.13 $\pm$ 1.56 \\ 
% \cmidrule[0.05em]{2-6}
\multirow{5}{*}{\emph{MESA}} & EEG-NET-SA & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx \\
& Mini-AIOSA & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx \\
& Mini-RRWaveNet & 68.59 $\pm$ 1.21 & 60.85 $\pm$ 0.82 & \textbf{63.38 $\pm$ 4.09} & 69.82 $\pm$ 1.92 \\ 
& DSepNet & \textbf{70.27 $\pm$ 1.25} & \textbf{61.59 $\pm$ 0.69} & 59.74 $\pm$ 4.27 & \textbf{72.75 $\pm$ 2.19} \\ 
& DSepEmbedder & 60.35 $\pm$ 0.85 & 47.35 $\pm$ 0.42 & 50.59 $\pm$ 3.03 & 61.50 $\pm$ 1.20 \\ 

\midrule[0.1em]

% \multirow{6}{*}{\emph{HeartBEAT}} & SVC & 60.68 $\pm$ 6.00 & 50.23 $\pm$ 3.02 & 56.27 $\pm$ 6.95 & 61.21 $\pm$ 7.81 \\ 
% & RF & 47.87 $\pm$ 2.56 & 45.00 $\pm$ 1.77 & \textbf{93.86 $\pm$ 0.93} & 40.67 $\pm$ 3.37 \\ 
% & XGB & 55.82 $\pm$ 2.64 & 49.40 $\pm$ 1.47 & 75.47 $\pm$ 0.72 & 52.73 $\pm$ 3.28 \\ 
% \cmidrule[0.05em]{2-6}

\multirow{5}{*}{\emph{HeartBEAT}} & EEG-NET-SA & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx \\
& Mini-AIOSA & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx & xx $\pm$ xx \\
& Mini-RRWaveNet & 49.63 $\pm$ 2.30 & 46.111 $\pm$ 1.37 & \textbf{90.36 $\pm$ 2.23} & 43.24 $\pm$ 3.14 \\ 
& DSepNet & 55.88 $\pm$ 3.60 & 49.26 $\pm$ 1.65 & 74.28 $\pm$ 4.07 & 52.92 $\pm$ 4.92 \\ 
& DSepEmbedder & 70.95 $\pm$ 1.40 & 49.91 $\pm$ 0.52 & 42.62 $\pm$ 0.94 & 73.16 $\pm$ 1.32 \\ 

\bottomrule[0.2em]
\end{tabular}
}
\label{table:exp3}
\end{table}

==> table/table_exp4.tex <==
\begin{table}[!t]
\caption{Subject-Independent Apnea Event Recognition with Fine-Tuning}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}

\toprule[0.2em]
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\begin{tabular}{@{}c@{}} \textbf{Finetuning} \\ \textbf{Sample Ratio}\end{tabular}} & 
\multicolumn{4}{c}{\textbf{Metrics}} \\
\cmidrule[0.1em]{3-6}
& & Accuracy & Macro F1 & Sensitivity & Specificity \\ 

\midrule[0.1em]

\multicolumn{6}{l}{\emph{MESA}} \\

\midrule[0.1em]

\multirow{4}{*}{Mini-RRWaveNet} & 0\% & 68.59 $\pm$ 1.21 & 60.85 $\pm$ 0.82 & \textbf{63.38 $\pm$ 4.09} & 69.82 $\pm$ 1.92 \\
& 5\% & 75.21 $\pm$ 0.83 & 60.97 $\pm$ 0.57 & 47.84 $\pm$ 19.49 & 80.34 $\pm$ 12.41 \\
& 10\% & 78.32 $\pm$ 1.11 & 64.37 $\pm$ 1.06 & 49.93 $\pm$ 15.24 & 83.57 $\pm$ 9.13 \\
& 20\% & \textbf{79.95 $\pm$ 0.31} & \textbf{67.17 $\pm$ 0.76} & 54.95 $\pm$ 14.49 & \textbf{84.44 $\pm$ 8.82} \\

\midrule[0.1em]

\multirow{4}{*}{DSepNet} & 0\% & 70.27 $\pm$ 1.25 & 61.59 $\pm$ 0.69 & 59.74 $\pm$ 4.27 & 72.75 $\pm$ 2.19 \\
& 5\% & 68.23 $\pm$ 0.52 & 58.83 $\pm$ 0.6 & 64.88 $\pm$ 12.96 & 68.30 $\pm$ 9.72 \\
& 10\% & 70.83 $\pm$ 0.77 & 61.21 $\pm$ 1.11 & \textbf{66.33 $\pm$ 10.33} & 71.38 $\pm$ 7.24 \\
& 20\% & \textbf{75.03 $\pm$ 0.33} & \textbf{64.59 $\pm$ 0.95} & 65.61 $\pm$ 10.25 & \textbf{76.62 $\pm$ 6.11} \\

\midrule[0.1em]

\multicolumn{6}{l}{\emph{HeartBEAT}} \\

\midrule[0.1em]

\multirow{4}{*}{Mini-RRWaveNet} & 0\% & 49.62 $\pm$ 2.30 & 46.11 $\pm$ 1.37 & \textbf{90.36 $\pm$ 2.23} & 43.24 $\pm$ 3.14 \\
& 5\% & 69.12 $\pm$ 1.54 & 56.93 $\pm$ 0.41 & 64.99 $\pm$ 20.49 & 68.83 $\pm$ 15.87 \\
& 10\% & \textbf{71.41 $\pm$ 2.73} & \textbf{59.56 $\pm$ 0.92} & 67.38 $\pm$ 17.34 & 71.76 $\pm$ 13.30 \\
& 20\% & 70.26 $\pm$ 2.18 & 59.39 $\pm$ 1.41 & 73.01 $\pm$ 17.00 & \textbf{69.99 $\pm$ 14.25} \\

\midrule[0.1em]

\multirow{4}{*}{DSepNet} & 0\% & 55.88 $\pm$ 3.60 & 49.26 $\pm$ 1.65 & \textbf{74.28 $\pm$ 4.07} & 52.92 $\pm$ 4.92 \\
& 5\% & 65.80 $\pm$ 3.30 & 54.49 $\pm$ 1.35 & 62.81 $\pm$ 15.78 & 65.87 $\pm$ 12.46 \\
& 10\% & 71.25 $\pm$ 1.11 & 58.34 $\pm$ 0.46 & 60.39 $\pm$ 14.06 & 72.61 $\pm$ 8.69 \\
& 20\% & \textbf{73.81 $\pm$ 1.98} & \textbf{60.58 $\pm$ 0.64} & 61.39 $\pm$ 13.73 & \textbf{75.28 $\pm$ 9.32} \\

\bottomrule[0.2em]
\end{tabular}
}
\label{table:exp4}
\end{table}

==> table/table_work_summary.tex <==
\begin{table*}[t]
\caption{A summary of the recent related works compared to our study}
\centering

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{tabular}{L{0.14\textwidth} C{0.04\textwidth} C{0.11\textwidth} C{0.07\textwidth} C{0.13\textwidth} C{0.1\textwidth} C{0.15\textwidth} C{0.07\textwidth}}

    \toprule[0.2em]
    
    \textbf{Study} & \textbf{Year} & \textbf{Dataset} & \textbf{\# Subjects} & \textbf{Nationality} & \textbf{Sensor Type} & \textbf{Features} & \textbf{Approach} \\ 
    
    \midrule[0.1em]
    
    Qi S. et al. \cite{9847226} & 2022 & Sun Yat-sen University & 92 & N/A & Wrist PPG & PRV & DL \\[0.4cm]

    Yibing C. et al. \cite{chen2021} & 2021 & Chinese PLA General Hospital & 83 & Chinese & Wrist PPG & PRV, \ch{SpO2} & ML \\[0.4cm]
    
    Remo L. et al. \cite{remo2020} & 2020 & UZ Leuven & 96 & Belgium & Finger PPG & DAP, \ch{SpO2} & ML \\[0.3cm]
    
    Gonzalo C. et al.\cite{gonzalo2019} & 2019 & Rio Hortega & 320 & Spanish & Finger PPG & Statistical non-linear measures, spectral features from \ch{SpO2} & ML \\
    
    \midrule[0.1em]

    Our work & 2023 & MESA* and HeartBEAT* & 241 and 281 & Black, White, Hispanic, Chinese, American & Finger PPG & PWA, PPI, derivative of PWA, derivative of PPI, SPD, DPD, PA & ML, DL \\
    
    % \multirow{2}{*}{Our work} & \multirow{2}{*}{2023} &MESA & 241 & Black, White, Hispanic, Chinese, American & \multirow{2}{*}{Finger PPG} & \multirow{2}{*}{PWA, PPI, Derivative of PWA, Derivative of PPI, SPD, DPD, PA} & \multirow{2}{*}{ML, DL} \\ 
    % & & HeartBEAT & 281 & American & & & & & \\
    
    \bottomrule[0.2em]
\end{tabular}

\vspace{0.5em}

\scriptsize{{\raggedright * Only MESA and HeartBEAT are publicly available datasets. \par}}

\vspace{0.5em}

\scriptsize{{\raggedright \textbf{Abbreviations:}
PRV; Pulse Rate Variability,
DAP; Decreases in the Amplitude fluctuation of PPG,
CVD; Cardiovascular Disease, 
DL; Deep Learning, 
ML; Machine Learning, 
PWA; Pulse Wave Amplitude,
PPI; Pulse to Pulse Interval,
SPD; Systolic Phase Duration,
DPD; Diastolic Phase Duration,
PA; Pulse Area\par}}
\end{table*}
